On Seven Fundamental Optimization Challenges in Machine Learning

Many recent successes of machine learning went hand in hand with advances in optimization. The exchange of ideas between these fields has worked both ways, with machine learning building on standard optimization procedures such as gradient descent, as well as with new directions in the optimization theory stemming from machine learning applications. In this thesis, we discuss new developments in optimization inspired by the needs and practice of machine learning, federated learning, and data science. In particular, we consider seven key challenges of mathematical optimization and develop a solution to each. Our first contribution is the resolution of a key open problem in Federated Learning: we establish the first theoretical guarantees for the famous Local SGD algorithm in the heterogeneous data regime. As the second challenge, we close the gap between the upper and lower bounds for the theory of two algorithms known as Random Reshuffling (RR) and Shuffle-Once that are widely used in practice, and set as the default data selection strategies for SGD in modern machine learning software. Our third contribution can be seen as a combination of our new theory for proximal RR and Local SGD yielding a new algorithm, which we call FedRR. Unlike Local SGD, FedRR can provably beat gradient descent in communication complexity in the heterogeneous data regime. The fourth challenge is related to the class of adaptive methods. In particular, we present the first parameter-free stepsize rule for gradient descent that provably works for any locally smooth convex objective. The fifth challenge is the development of an algorithm for distributed optimization with quantized updates that preserves linear convergence of gradient descent. Finally, in our sixth and seventh challenges, we develop new VR mechanisms applicable to the non-smooth setting based on proximal operators.

==> parts/notation_table.tex <==
%\refstepcounter{chapter}%
\begingroup
\let\clearpage\relax
\chapter{ Tables of Frequently Used Notation}\label{sec:table}
\endgroup



\renewcommand{\EE}{\mathbb{E}}


{
\footnotesize



 \begin{longtable}[H]{| p{.20\textwidth} | p{.80\textwidth}| } 
 \caption{Summary of frequently used notation.}\label{tbl:notation}\\
\hline
\multicolumn{2}{|c|}{{\bf \normalsize For all chapters} }\\
\hline
\multicolumn{2}{|c|}{ Basic }\\
\hline
$k$ & Iteration/epoch counter \\
$\E{\cdot}$& Expectation\\
$\EE_\xi\left[\cdot\right]$& Expectation with respect to the variable $\xi$ \\
$\EE_k\left[\cdot\right]$& Expectation conditioned on the information up to iteration $k$ \\
$\langle \cdot ,\cdot \rangle$,  $\| \cdot \|$ & Standard inner product and norm in $\R^d$ $\langle x ,y \rangle =\sum_{i=1}^d x_iy_i$; $\| x \| =\sqrt{\langle x ,x \rangle} $ \\
$\ell_p$ norm & $\|x\|_p= \left(\sum_{l=1}^d x_l^p \right)^{\frac{1}{p}}$, $p\in [1, +\infty]$ \\
$\lambda_{\min} (\cdot), \lambda_{\min}^+(\cdot)$ & The smallest and the smallest positive eigenvalues of a matrix   \\
$\lambda_{\max}(\cdot)$ & The largest eigenvalue of a matrix   \\
$\nabla h(x)$& Gradient of a differentiable function $h$ \\
$\nabla^2 h(x)$& The Hessian of a twice differentiable function $h$  \\
\hline
\multicolumn{2}{|c|}{ Objective }\\
\hline
	$P$ & Full objective if there is a non-smooth term\\
	$d$ & Dimension of the primal space $x\in \RR^d$  \\
	$f\colon \R^d \rightarrow \R$ & Smooth part of the objective \\
    $f_j\colon \R^d \rightarrow \R$ & Differentiable function ($1\leq j \leq n$) if finite-sum setting \\
    $f(\cdot; \xi)\colon \R^d \rightarrow \R$ & Almost-surely differentiable function in expectation setting \\
    $n$ & Number of samples in finite-sum setting \\
    $M$ & Number of nodes in parallel setting \\
	$\psi\colon \R^d \rightarrow \R \cup \{\infty \}$ & Non-smooth part of the objective (proper, closed, convex)\\
	$x^\star$ & Global optimum\\
	$L$ & (Global) smoothness constant of $f$ \\
	$\mu$ & Strong convexity constant  \\
	$\kappa$  & The condition number $\kappa = L/\mu$ for strongly convex objectives \\
  \hline
\multicolumn{2}{|c|}{ Other }\\
\hline
     $[n]$ & Set $\{1,2,\dots,n\}$ \\
     $D_h(x,y)$ & Bregman distance $D_h(x,y) = h(x) - h(y)-\langle \nabla h(y),x-y \rangle$ \\
	$\dom(h)$ & Domain of $h$, $\dom (h) = \{x\;:\; h(x)<+\infty\} $ \\
	$\partial h$ & Subdifferential of $h$, $\partial h(x)= \{s \;:\; h(y) \geq h(x) + \langle s, y-x \rangle\}$, $x\in \dom(h)$ \\
	$\prox_{\gamma h}(x)$ & Proximal operator of a function $h$, $\prox_{\gamma hi}(x) = \argmin_{u} \left\{h(u) + \frac{1}{2\gamma}\|u - x\|^2 \right\}$ \\ 
	$\gamma$ & Fixed stepsize \\
	$\gamma_k$ & Stepsize at iteration $k$ \\
\hline
\end{longtable}


%%%%%%%%%%%%% LOCAL SGD


\begin{longtable}{| p{.20\textwidth} | p{.80\textwidth}| } 
 \caption{Notation specific to Chapter~\ref{chapter:local_sgd}.}\label{tab:notation-summary}\\
\hline
\multicolumn{2}{|c|}{{\bf \normalsize Chapter~\ref{chapter:local_sgd}} }\\
\hline
    $g^k_m$ & Stochastic gradient at time $k$ on node $m$  \\ 
    $x^k_m$ & Local iterate at time $k$ on node $m$ \\ 
    $g^k$ & The average of stochastic gradients across nodes at time $k$  \\ 
    $\bar{g}^k$ & Expected value of $g^k$, $\ec{g^k} = \bar{g}^k$ \\ 
    $\hat{x}^k$ & The average of all local iterates at time $k$ \\ 
    $r^{k}$ & The deviation of the average iterate from the optimum $\hat{x}^k - x^\ast$ at time $k$ \\ 
    $\sigma^2$ & Global uniform bound on the variance of the stochastic gradients for identical data   \\ 
    $\sigmaopt^2$ & The variance of the stochastic gradients at the optimum  for identical data \\ 
    $\sigmaf^2$ & The variance of the stochastic gradients at the optimum  for heterogeneous data \\ 
    $k_1, k_2, \ldots, k_p$ & Timesteps at which synchronization happens in \algname{Local SGD} \\ 
    $H$ & Maximum number of local steps between communications, $H=\max_{p} \abs{k_p - k_{p+1}} $   \\ \hline
\end{longtable}


%%%%%%%%%%%%% RR

\begin{longtable}{| p{.20\textwidth} | p{.80\textwidth}| } 
 \caption{Notation specific to Chapters~\ref{chapter:rr} and \ref{chapter:proxrr}.}\label{tab:notation}\\
  \hline
  \multicolumn{2}{|c|}{{\bf \normalsize Chapters~\ref{chapter:rr} and~\ref{chapter:proxrr}} }\\
  \hline
  $\pi$ &
    \begin{tabular}[l]{@{}l@{}}A permutation $\pi = \br{ \prm{0}, \prm{1}, \ldots, \prm{n-1} }$ of $\{ 1, 2, \ldots, n \}$ \\ Fixed for \algname{Shuffle-Once} and resampled every epoch for \algname{Random Reshuffling}.\end{tabular} \\
  $x^k_i$              & The current iterate after $i$ steps in epoch $k$, for $0 \leq i \leq n$                                                                       \\ 
  $g^k$                & The sum of gradients used over epoch $k$ such that $x^{k+1}=x^k-\gamma g^k$                                                                                                      \\ 
  $\sigma_{k}^2$       & The variance of the individual loss gradients from the average loss at point $x^k$                                                            \\ 
  $A, B$ & Assumption~\ref{asm:2nd-moment} constants                                                                                                  \\
  $\delta_{k}$         & Functional suboptimality, $\delta_{k} = f(x^k) - f^\ast$, where $f^\ast= \inf_{x} f(x)$ \\ 
  $r_{k}$              & The squared iterate distance from an optimum for convex losses $r_{k} = \sqn{x^k - x^\ast}$       \\ \hline
\end{longtable}




%%%%%%%%%%%%%%% Adaptive

\begin{longtable}{| p{.20\textwidth} | p{.80\textwidth}| } 
 \caption{Notation specific to Chapter~\ref{chapter:adaptive}.}\\
\hline
\multicolumn{2}{|c|}{{\bf \normalsize Chapter~\ref{chapter:adaptive}} }\\
\hline
$L_k $ & Estimated gradient Lipschitz constant \\
$\gamma_k $ & Adaptive stepsize \\
$\mu_k $ & Estimated strong convexity \\
$\theta_k $ & Stepsize ratio, $\theta_k = \frac{\gamma_k}{\gamma_{k-1}}$ \\
$\Theta_k $ & Strong convexity ratio, $\Theta_k = \frac{\mu_k}{\mu_{k-1}}$ \\
$\beta_k $ & Estimated momentum \\
$w_i $ & The weight of $x^i$ in the ergodic iterate $\hat x^K$ \\
$\Psi^k$ & Lyapunov function \\
\hline
\end{longtable}




%%%%%%%%%%%%%%% DIANA

\begin{longtable}{| p{.20\textwidth} | p{.80\textwidth}| } 
 \caption{Notation specific to Chapter~\ref{chapter:diana}.}\label{tbl:notation-table}\\
\hline
\multicolumn{2}{|c|}{{\bf \normalsize Chapter~\ref{chapter:diana}} }\\
\hline
$\sign(t)$ & The sign of $t$  ($-1$ if $t < 0$, $0$ if $t=0$ and $1$ if $t>1$) \\
$x_{(j)}$ & The $j$-th element of $x\in\R^d$\\
%$\|x\|_0$ & Number of nonzero elements of $x$ \\
$g_i^k$ & Stochastic gradient at time $k$ on node $i$  \\
$g^k$ & The average of stochastic gradients across nodes at time $k$ \\ 
$\sigma_i^2$ & Variance of the stochastic gradient $g_i^k$  \\
$\sigma^2$ & Variance of the stochastic gradient $g^k$ \\ 
$h_i^k$ & Stochastic approximation of $\nabla f_i(x^\star)$  \\
$\Delta_i^k$ & $\Delta_i^k = g_i^k - h_i^k$ \\
$\text{Quant}_p(\Delta)$ & Full $p$-quantization of vector $\Delta$ \\
$d_l$ & Size of the $l$-th block for quantization \\ 
$m$ & Number of blocks for quantization\\
$\beta$ & Momentum parameter \\
$\hat \Delta_i^k$& Block $p$-quantization of $\Delta_i^k = g_i^k - h_i^k$ \\
$\hat \Delta$ & $\hat \Delta^k = \frac{1}{M}\sumiM\hat\Delta_i^k$  \\ 
$\hat g_i^k$ & Stochastic approximation of $\nabla f_i(x^k)$ \\
$\hat g^k$ & $g^k = \frac{1}{M}\sumiM g_i^k$ \\
$v^k$ & Stochastic gradient with momentum $v^k = \beta v^{k-1} + \hat g^k$\\
$h^{k}$ & $h^{k} = \frac{1}{M}\sumiM h_i^{k}$ \\
$\Psi_l(x)$ & Variance of the $l$-th block $\Psi_l(x) = \|x(l)\|_1\|x(l)\|_p - \|x(l)\|^2$ \\
$\Psi(x)$ & Variance of the quantized vector $\Psi(x) = \sum\limits_{l=1}^m\Psi_l(x)$ \\
$\widetilde d$ & $\widetilde d = \max\limits_{l=1,\ldots,m}d_l$ \\
$\alpha_p$ & $\alpha_p = \alpha_p(\widetilde d)$ \\
$h_i^\star$ & $h_i^\star = \nabla f_i(x^\star)$  \\
$V^k$ & Lyapunov function $V^k = \|x^k - x^\star\|^2 + \frac{c\gamma^2}{M}\sumiM\|h_i^k - h_i^\star\|$  \\
$\zeta$ & Data dissimilarity, $\frac{1}{M}\sum_{i=1}^M\|\nabla f_i(x) - \nabla f(x)\|^2 \le \zeta^2$ \\
$\mathbb{E}_{Q^k} \left[ \cdot \right]$ & Expectation with respect to quantization  \\
\hline
\end{longtable}


%%%%%%%%%%%%%%% SDM

\begin{longtable}{| p{.20\textwidth} | p{.80\textwidth}| } 
 \caption{Notation specific to Chapter~\ref{chapter:sdm}.}\label{tbl:notation_sdm}\\
\hline
\multicolumn{2}{|c|}{{\bf \normalsize Chapter~\ref{chapter:sdm}} }\\
\hline
$\cX^\star $ & Set of optimal solutions $\cX^\star = \{x^\star\in \RR^d \;:\; P(x) \geq P(x^\star) \; \forall x\in \RR^d\}$ \\
$\sigma_{\star}^2$ & Gradient noise at optimum $\sigma_{\star}^2= \EE_\xi \left[\|\nabla f(x^\star; \xi) - \nabla f(x^\star)\|^2 \right]$ \\
$g$ & $g(x) = \frac{1}{m}\sum \limits_{j=1}^m g_j(x)$  (proper, closed, convex)\\
$g_j$ & $g_j\colon\RR^d\to \RR\cup \{+\infty\}$ (proper, closed, convex)\\
$\phi_j$ & Structured form of $g_j$ $g_j(x) = \phi_j(\mA_j^\top x)$, $\mA_j\in \RR^{d\times d_j}$ \\
$v^k$ & Estimator of $\nabla f(x^k)$ \\
$y_1^k,\dots,y_j^k $ & Dual variables \\
$p_j$ & Probability of selecting index $j$ \\
$\gamma$ & Stepsize associated with $f$ and $\psi$ \\
$\eta_j$  & Stepsize associated with $g_j$,  $\eta_j = \frac{\gamma}{m p_j}$ \\
$\cL^k$ & Lyapunov function   $\cL^k
        =  \ec{\|x^k - x^\star\|^2} + \cM^k + \cY^k$ \\
$\cY^k$ & Dual distance to solution $ \cY^k
	= (1+\nu)\sumlm \eta_l^2\ec{\|y_l^{k} - y_l^\star\|^2}$\\      
$L_j$ & Smoothness constant of $g_j$, $L_j\in\RR\cup \{+\infty\}$ ($L_j=+\infty$ if $g_j$ is non-smooth)\\
$\nu$	& $\nu = \min_{j=1,\dots,m} \frac{1}{\eta_j L_j}$ ($\nu=0$ if any $g_j$ is non-smooth)  \\
$\ind_{\cC}(x)$ & Characteristic function of a set $\cC$, $\ind_{\cC}(x)= \begin{cases}0 & x\in \cC \\ +\infty & x\notin \cC\end{cases}$ \\
$\Pi_{\cC}(x)$ & Projection onto a set $\cC$, $\Pi_{\cC}(x) =  \prox_{\ind_{\cC}}(x)= \argmin_{u\in \cC} \|u-x\|$ \\
\hline
\end{longtable}

%%%%%%%%%%%%%%% PDDY

\begin{longtable}{| p{.20\textwidth} | p{.80\textwidth}| } 
 \caption{Notation specific to Chapter~\ref{chapter:pddy}.}\\
\hline
\multicolumn{2}{|c|}{{\bf \normalsize Chapter~\ref{chapter:pddy}} }\\
\hline
$\mL $ & Linear operator from the objective \\
$\cX $ & Primal space \\
$\cY $ & Dual space \\
$\cL\colon \cX\times \cY\to \R $ & Lagrangian function \\
$y^\star$ & Dual solution \\
$\tau$ & Dual stepsize \\
$\mP$ & Linear operator that defines the primal-dual metric \\
$(\Omega,\cF,(\cF_k)_k,\bP)$ & Probability space \\
$V^k$ & Lyapunov function \\
\hline
\end{longtable}



}







==> rr_prox/algs/proxrr.tex <==
\begin{algorithm}[t]
    \caption{Proximal Random Reshuffling (\rrbox(ProxRR})}
    \label{alg:proxrr}
    \begin{algorithmic}[1]
    \Require Stepsizes $\gamma_k > 0$, initial vector $x^0 \in \R^d$, numbers of epochs $T$
        \For{epochs $k=0,1,\dotsc,T-1$}
            \State Sample a permutation $\prm{0}, \ldots, \prm{n-1}$ of $\{ 1, 2, \ldots, n \}$
            \State $x^k_0 = x^k$
            \For{$i=0, 1, \ldots, n-1$}
                \State $x^{k}_{i+1} = x^k_{i} - \gamma_k \nabla f_{\prm{i}} (x^k_i)$
            \EndFor
        \State $x_{k+1} = \prox_{\gamma_k n \psi}(x^{k}_{n})$
        \EndFor
    \end{algorithmic}
\end{algorithm}

